Prompting in the Dark: Assessing Human Performance in Prompt Engineering for Data Labeling When Gold Labels Are Absent

Millions of users prompt large language models (LLMs) for various tasks, but how good are people at prompt engineering? Do users actually get closer to their desired outcome over multiple iterations of their prompts? These questions are crucial when no gold-standard labels are available to measure progress. This paper investigates a scenario in LLM-powered data labeling, "prompting in the dark," where users iteratively prompt LLMs to label data without using manually-labeled benchmarks. We developed PromptingSheet, a Google Sheets add-on that enables users to compose, revise, and iteratively label data through spreadsheets. Through a study with 20 participants, we found that prompting in the dark was highly unreliable -- only 9 participants improved labeling accuracy after four or more iterations. Automated prompt optimization tools like DSPy also struggled when few gold labels were available. Our findings highlight the importance of gold labels and the needs, as well as the risks, of automated support in human prompt engineering, providing insights for future tool design.

==> Figures/Figure-System-Interface.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Interfaces/System-Interface-1.jpeg}
    \caption{\textbf{Initialize System:} PromptingSheet utilizes four tabs for system initialization: (A) Dataset, (B) Context, (C) Rule Book, and (D) Shots. Users begin by importing data to the ``Dataset'' tab and clicking the ``Index Data ID'' button to index data instances. The ``Context'', ``Rule Book'', and ``Shots'' are three key components that users can configure to guide LLMs. After data importing, users answer questions related to task instruction in the ``Context'' tab, which will later be provided to LLMs. Next, users will navigate to the ``Rule Book'' tab to define annotation labels with rules. Optionally, users may add gold shots in the ``Shots'' tab, which can serve as reference examples for LLMs.}
    \label{fig:system-interface-1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{Figures/Interfaces/System-Interface-2.jpeg}
    \caption{\textbf{Sampling Data:} User can use Random or Sequential Sampling to sample data instances. The sampled data instances will be copied to the ``Working Data Sample'' tab from the ``Dataset'' tab. PromptingSheet will only annotate data instances from the ``Working Data Sample'' tab.}
    \label{fig:system-interface-2}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Interfaces/System-Interface-3.jpeg}
    \caption{\textbf{Data Annotation: }Users proceed to click the ``Start Annotation'' to annotate data instances from the ``Working Data Sample'' tab. The annotation results will be saved to a new tab. The new tab contains the basic data instance information (Data ID, Group ID, and Data instance), LLM Label, LLM Explanation (if checked the ``Explanation'' checkbox), and Human verification columns (``I agree with the LLM Label'' Checkbox, Human Label, ``Gold Shot'' Checkbox, Human Explanation for note, ``Keep it in the next data sample'' Checkbox, Labeling Cost). }
    \label{fig:system-interface-3}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{Figures/Interfaces/System-Interface-4.jpeg}
    \caption{\textbf{Verification and Iteration: } During the verification process, users can confirm with LLM labels or input their own labels (A), select gold shots (B1), and select data instances for re-annotation (C1). 
    In the iteration process, 
    users can click the ``Add Shots'' button (B2) to add the selected gold shots to the ``Shots'' tab (B3). 
    Additionally, users can click the ``Add Back'' button (C2) to add the selected data instances to the ``Working Data Sample'' tab (C3) for re-annotation.}
    \label{fig:system-interface-4}
\end{figure}


==> Sections/2-4-survey-data-annotation.tex <==
\steven{
We conducted a survey study to investigate how individuals interact with LLMs and utilize gold-standard labels in the data annotation process. 
The participants primarily represent roles in research, machine learning engineering, and software development. \\
\textbf{Workflows: }Participants described diverse workflows for integrating LLMs into data annotation process, highlighting a common iterative and human-in-the-loop approach. \textbf{Most workflows begin with manual annotation of a small subset of data to establish a baseline.} Participants then employ prompt engineering, iteratively refining LLM prompts by evaluating their performance against the manually annotated subset. \\
Once refined, the prompts are used to label larger datasets, with participants using tools or manual checks to review the LLM's annotations and identify any invalid labels. The process is typically concluded with a thorough manual verification of the dataset. \\
One participant mentioned they manually tabulate data points along with their descriptions. \\
\textbf{Initialize Prompting: }Most participants use their pre-defined prompts to initialized the annotation on their known tasks. 
For new tasks, one participant mentioned that they initialize the annotation process with LLMs by starting with a clear problem definition and iteratively refining a classification-based approach. For less familiar tasks, some participants may seek suggestions from the LLM to guide the initial setup.
\textbf{Revising Prompt: } Participants use a small dataset to finetune the prompt. They address issues by adding rules or context examples to tackle failure cases. When inconsistencies or error arise, they revisit and recheck the manually tagged dataset to improve performance. Some participants also engage the LLM by asking questions about data points and their descriptions, retraining to against inconsistencies to minimize hallucinations and enhance annotation reliability.
}

==> Sections/2-6-explaination-data-annotation.tex <==
Explanations in AI models play a critical role in enhancing user comprehension, offering valuable insights, and improving the usability of AI-assisted tools across a range of tasks, including deception detection and UX evaluation~\cite{lai2019human, fan2022human}. While prior studies have primarily investigated tasks with predefined standards, our research focuses on a dynamic context where task standards evolve iteratively through user interactions with the system.
Building on existing work, prior studies have emphasized the importance of fostering human-AI synergy by envisioning a collaborative relationship where humans and AI function as team players~\cite{lai2020chicago,fan2022human}.
However, human-AI collaboration often introduces challenges such as overreliance -- when humans uncritically accept incorrect AI recommendations~\cite{passi2022overreliance, buccinca2021trust}. These studies propose several strategies to mitigate overreliance, including employing cognitive forcing functions, improving clarity in communication, and providing informative explanations.
Notably, \citet{vasconcelos2023explanations} illustrated that overreliance on AI is not an inherent cognitive bias but rather a strategic decision shaped by the perceived costs and benefits of engaging with AI explanations. Their research revealed that overreliance can be alleviated by increasing task complexity, enhancing the clarity of AI explanations, or reducing the incentives for reliance.
These insights underscore the importance of designing AI explanations that effectively balance user trust and scrutiny.
In contrast to all these studies, which typically examine end users completing tasks using AI-generated explanations, our study focuses on requesters as the primary users, who are inherently accountable for their tasks and possess personalized or domain-specific expertise. 
Unlike the straightforward application of LLM explanations to perform tasks, we explore the underexplored impact of these explanations on requesters' decision-making processes and their ability to guide task pipelines effectively. 
We aim to determine whether the presence of LLM explanations influences requesters’ capacity to effectively direct LLMs in labeling tasks.

\steven{\citet{vasconcelos2023explanations} demonstrated that overreliance on AI is not an inherent cognitive bias but rather a strategic decision influenced by the perceived costs and benefits of engaging with AI explanations. 
Their study showed that overreliance can be mitigated by increasing task difficulty, improving the comprehensibility of AI explanations, or decreasing incentives for reliance.
In our study, we focus on requesters as the target users, who are inherently responsible for their tasks.
Rather than solely using LLM explanations for task completion, we want to investigate whether the existence of explanations could impact users' ability to effectively guide LLM in labeling task. 
}

\steven{\citet{mueller2019explanation} mentioned that effective explanations can enhance user comprehension and provide actionable insights. 
They also noted that aligning explanations with users’ mental models facilitates a clearer understanding of the system’s logic and behavior.
To foster collaboration, AI systems should act as team players, building shared understanding with users. 
Building on these insights, we aim to explore how users leverage explanations to better guide LLMs, aligning them with their standards and expectations. }

\steven{\citet{lai2019human} highlighted  the importance of transparency in ML models on deception detection tasks. 
Based on this, \citet{lai2020chicago} proposed future directions for developing human-centered tutorials and explanations to foster synergy between humans and AI.  
In their work, explanations were generated using feature-based, example-based, and human-text approaches. While feature-based and example-based methods often lack transparency, human-text explanations, derived by summarizing scientific studies and paraphrasing them into human-readable rules, face scalability limitations.
The advent of LLMs allows us provide more comprehensive and transparent explanations to users.
We seek to investigate whether this enhanced transparency can significantly impact users’ ability to guide LLMs effectively and align their outputs with user-defined standards.}

\steven{\citet{fan2022human} demonstrated that explanations significantly enhance UX evaluators’ understanding of AI decisions, particularly in identifying usability problems.
They highlighted that explanations play a pivotal role in improving the usability of AI-assisted tools for UX evaluation. 
Unlike their study, which focused on tasks with pre-set standards, our investigation explores a dynamic context where task standards evolve iteratively through user interactions with the system. Here, we aim to understand how explanations can support the development of new standards in such iterative processes.}

\steven{While previous studies have explored how explanations can enhance human performance from the labeler’s perspective, our study focuses on the requester’s viewpoint, which remains an underexplored area requiring further investigation.}

==> Sections/2-7-variable-selection.tex <==
There are lots of variables in a system could impact user's performance. 
\citet{kulesza2012tell} suggested that the more users understand the underlying system, the more effectively they can control it. 

\steven{\citet{lee2024clarify} introduces a system that allows non-expert users to train and correct models by directly interact with model using natural languages. In each iteration, the system will use similarity score between user description and image and display images above a threshold. The system will also provide 0-1 score indicating how well description separates the error cases from the correct prediction. Basically using metrics to guide user.
It does not mentioned about the sample size selection.}

\steven{[Data Instance:] In active learning, the goal is to minimize the amount of interaction required by users by querying the most important information~\cite{bernard2018vial}. [This can be used to justify why we increase to 50, to ensure the diversity. We cannot deploy algorithms to find most representative data sample because of the technical limitation of Google App Script]}

\steven{[Data Instance:] \citet{vermetten2022analyzing} investigated how the number of sample size affects the reliability of algorithm comparisons in iterative optimization. The study found that small sample sizes lead to high variability in performance estimates and larger sample sizes could decrease the impact of outliers. The performance could loss due to small samples and increasing sample size consistently improves reliability. }

\steven{\citet{purohit2018ranking} suggested capping the maximum number of annotation tasks assigned per unit of time to manage workload effectively to mitigate annotator burnout.}

\steven{\citet{pandey2022modeling} mentioned annotator can develop a mental representation of a concept by seeing a sufficient number of examples.}

\steven{\citet{wang2016human} limited users to verify the top-50 in each round, where users did binary classification on whether image was match or not.}

\steven{[explanation]\citet{kulesza2015principles} presents a system that explains the reason behind each prediction for users to better understand the system's logic to tailor the system toward their needs. In the system, users will modify feature weights within the model. n our LLM-powered system, users need to use natural language to guide the system. However, this can be more challenging because large models are less responsive to prompt variations compared to smaller models~\cite{zhuo2024prosa}.}

\steven{The more users understand the underlying system, the more effectively they can control it~\cite{kulesza2012tell}.}

\steven{\citet{teso2023leveraging} discusses a general framework for incorporating explanations into interactive machine learning. Users can get a better understanding of the machine's logic by observing the machine's explanations. [In LLM system, the explanation is the supporting argument for selecting a label.] Once understanding the bugs and limitation, users could modify the algorithm to correct flaws~\cite{kulesza2015principles}. [In our case, user cannot directly modify LLMs but only provide natural language to guide them. Also, subjective tasks does not have universal correct answers, where users need to provide their own standards to steer LLMs. ] }

\steven{[Task Difficulty:] 
A task being too difficult can frustrate users~\cite{zheng2022virtual}, particularly when exceeding their skill level, and a task being to easy can lead to boredom~\cite{zhang2021personalized}.
  These study focused on the impacts of difficulty on users' performance on a pre-defined task. However, in our study, our work prioritizes the dynamics of human-LLM interaction, emphasizing how effective humans could guide LLMs to align with their standard. In this context, the difficulty level of the task itself is less critical, as our primary objective is to assess the effectiveness of human guidance, regardless of the inherent complexity of the task.}


\steven{[task type:]\citet{cayir2016study} found the complexity and definition of a task significantly influence user performance. }

\steven{[task type:] \citet{hettiachchi2022survey} discusses different task assignment methods, including the modeling of worker performance and the impact of task heterogeneity on assignment strategies.
\citet{zhen2021crowdsourcing} provides a detailed exploration of task assignment challenges, task types, and their effects on worker performance and task outcomes. 
}

==> Sections/deleted/3-3-0-workflow-step-0.tex <==

To begin using \system, users start with an empty Google Sheet and turn on the add-on. The system will automatically initialize necessary tabs for users, and the add-on interface will be displayed on the right side of the spreadsheet. 

\subsubsection{System Setup}



\paragraph{Setup Dataset} 
Users can import their data instances with `Group ID' into the ``Dataset'' tab and click ``Index Data ID''. \system will then assign unique data IDs to each data instance under the `Data ID' column.

\paragraph{Two Data Instance Formats Handling}\steven{I kind of want to make this explanation attached to the workflow and do not want it to be parallel with the workflow. It is the description of the system}



%\kenneth{Load data, index data, and sample data (NOT optional) --- mention 10 vs 50 data study}

==> Sections/deleted/3-3-1-workflow-step-1.tex <==


\kenneth{Three parts of the prompt}
%\subsubsection{Compose/Refine the prompt}
This step is the core element of the system, allowing users to create and modify prompts for their annotation tasks. In the ``Context'' tab, users need to answer questions about the data annotation task to provide task context to LLMs. Then, they will navigate to the ``Rule Book'' tab to add annotation labels with corresponding definitions. This procedure is mandatory as it supplies both label classes and rules that the LLMs will adhere to. Afterward, users can add instances with their gold labels, which will serve as examples from which the LLMs can learn. 
This step is optional in the first iteration, as users may not yet have a well-defined gold standard. As they review more data instances, they can identify additional instances that could serve as gold standard references for the LLMs.
Users can modify these three sections at any time in future iterations.

==> Sections/deleted/3-3-2-workflow-step-2.tex <==
\kenneth{Keep the sample}



%\subsubsection{Sample/Resample a random subset}

Users can randomly or sequentially sample data into the `Working Data Sample' tab. With Random Sample, users enter any whole number between 1 and the total number of the group IDs in the whole dataset. \system will then randomly select that number of groups from the dataset and copy them into the ``Working Data Sample'' tab. 
In Sequential Sample, users specify a range of group IDs, and \system will then import the data instances from the selected range of groups into the ``Working Data Sample'' tab.
Once the sampling starts, all data instances in the ``Working Data Sample' tab will be removed except ones that have `Keep it in the next data sample'' checked. 

\paragraph{Keep it in the next data sample} For instances that have ``Keep it in the next data sample'' checked, their group will remain in the later random or sequential sampling.

\paragraph{Annotation Note} Only the data instances in the ``Working Data Sample'' tab will be annotated once the ``Start Annotation'' button is clicked.

==> Sections/deleted/3-3-3-workflow-step-3.tex <==
\kenneth{also mention explanation study}



%\subsubsection{Use the prompt to label the data sample}
After finalizing the prompt tabs (``Context'', ``Rule Book'', and ``Shots'') and sampling data instances, users can click on the ``Start Annotation'' button to annotate all instances in the ``Working Data Sample'' tab. 
On the backend, \system gathers all questions and answers from the ``Context'' tab and inputs them into GPT-4o to generate an instruction prompt.
The system then combines this prompt with rules and the provided gold shots to create a final annotation prompt.
For each data group, the system sends one request to GPT-4o using this final prompt for annotation.
After receiving the LLM's output, the system parses the results and updates the spreadsheet with the annotated information for each instance.

Before clicking the ``Start Annotation'' button, users can choose whether to display the LLM explanation in the annotation results. To evaluate the impact of LLM explanations on users' prompt performance, our user study participants were randomly divided into two equal groups: one group had the option to display the LLM explanation, and the other group did not have access to it.\steven{explanation study}

==> Sections/deleted/3-3-4-workflow-step-4.tex <==
%\subsubsection{Observe and revise the prompt}
The annotation results will be saved to a new task tab. Users can start verifying LLM labels. Users who disagree with an LLM label can assign a new human-generated label to the data instance under the ``Human Label'' column. If users find good examples that can be used for later LLM learning, they can check the ``Gold Shot'' checkboxes. They can also check the ``Keep it in the next data sample'' checkboxes if they want to re-annotate data instances.

If users are not satisfied with the annotated results, they can refine the prompt tabs by modifying the ``Context'' answers, updating ``Rule Book'' definitions, and adding gold standard examples to the ``Shots'' tab. 


%\subsubsection{Iterations}
During the Observation process, users can check the ``Keep it in the next data sample'' checkboxes for data instances they want to re-annotate in the next iteration. Once the process is complete, they can click the ‘Add Back’ button to copy these instances to the ``Working Data Sample'' tab.  
From there, they can re-sample or re-use instances for the next iteration.


==> Sections/deleted/4-2-DSPy-process.tex <==






In our study, we tried a wide a range of prompt refining algorithms from DSPy to get the best performing prompt for each user iteration.
We started with a Simple Prompt approach, that uses the abstract prompts constructed by DSPy. This approach employs the simplest DSPy teleprompter, BootstrapFewShots, to generate optimized examples using all the few-shot examples annotated by the user during the experiment. Thus, essentially optimizing the prompts using few-shot learning.


Apart from the Simple Prompt approach, we also evaluated other teleprompters offered by DSPy namely, BootstrapFewShot, MIPRO and COPRO. For these optimizers we used the initial task instructions, label definitions and few shot examples provided by the user for each iteration. The BootstrapFewShots teleprompter automatically generates to include in the user defined prompt based on the few-shot examples provided. 
The COPRO teleprompter focuses on optimizing the prompt instructions themselves while keeping the few shot examples constant. This allows for generating more optimized prompt instructions even in the absence of labeled examples.
The final teleprompter we tried was the MIPRO. MIPRO is a combination of both COPRO and BootstrapFewShot teleprompters in the sense that it does prompt refining as well as generates optimized examples using the few-shot examples provided. 




In this manner, we have investigated how optimizing different parts of the prompt has effects on the performance.

==> Sections/deleted/5-1-1-experimental-results-pure-participants.tex <==



%\paragraph{Not accessing LLM Explanations and exploring more instances per iteration help participants on PITD}
 % Which setting helps participants on PITD?

%We further examined the effects of \textbf{LLM Explanation Access} and \textbf{the number of data instances per iteration}. 





%\paragraph{Does LLM Explanation Helps?}









% \steven{The following can only show that participants under that certain group had a higher ACC or lower MSE. It does not reflect the impact of our system.}
% In single conditions (Table~\ref{tab:single-condition-t-test}), focusing participants within one condition, \textbf{LY} participants achieved notably higher accuracy compared to LN and 50Y participants. 
% In addition, \textbf{LY} participants demonstrated significantly lower MSE than all other participants. 

% In the mixed conditions (Table~\ref{tab:mixed-condition-t-test}), which combined access to LLM explanation with exploring 50 instances per iteration conditions, LN-50Y participants showed a significantly lower accuracy than the rest of the conditions. 
% LY-50Y participants had significantly lower MSE than other participants, except LY-50N participants.




==> Sections/deleted/5-1-2-experimental-result-with-DSPy.tex <==
The previous section showed only certain settings could help participants on improving prompt performance. It would be interesting to explore the potential impacts of using an automatic prompt optimizing tool, such as DSPy~\cite{khattab2023dspy}, to assist with refinement. 


We then analyzed the DSPy fine-tuned prompts under different conditions in Table~\ref{tab:dspy-general-conditions-t-test}. LN-50Y demonstrated a significantly higher labeling accuracy improvement than other conditions, while LN-50N showed a significant drop in accuracy. In terms of MSE, both LY-50Y and LY-50N showed significant declines in MSE than LN-50Y and LN-50N. 

We further narrowed it down into different conditions for each DSPy algorithm in Table~\ref{tab:dspy-all-conditions-t-test}. For Bootstrap, LN-50N dropped the accuracy significantly than LY-50Y and LN-50Y. LY-50Y demonstrated a significant drop in MSE compared to LN-50Y and LN-50N. 
For Simple Prompt, LN-50N performed a significant dropping in labeling accuracy compared to other conditions, and LY-50Y had a significant drop in MSE compared to the rest of the conditions.  
For Mipro, LY-50Y showed a significant improvement in labeling accuracy compared to LY-50N and LN-50N. LN-50Y showed a notable improvement in accuracy over LN-50N and also achieved a significantly better MSE improvement compared to both LY-50Y and LY-50N.
In Copro, there was no significant difference between conditions for labeling accuracy. As for MSE, LY-50N exhibited a significant drop in conditions including LN, and LN-50N demonstrated a significant improvement in conditions containing LY.

In summary, DSPy algorithms demonstrated a greater improvement in accuracy and MSE for participants who \textbf{did not access the LLM explanation}. DSPy optimizers were more effective in helping participants with 50 instances per iteration enhance labeling accuracy, while participants reviewing fewer instances per round saw a more pronounced improvement in MSE. 

\input{Tables/dspy-t-test/dspy-t-test-general-condition}


% DSPy improved labeling accuracy on average for LN-50Y participants and consistently enhanced MSE when the Mipro and Copro optimizers were applied. 
% Interestingly, for participants under the LN-50N condition, DSPy worsened accuracy but contributed to the highest improvement in MSE.
% Overall, DSPy performed the best on prompting refinement on LN-50Y.
\begin{figure}
    \centering
    \begin{subfigure}{0.85\textwidth}
    \includegraphics[width=\linewidth]{Figures/Results/Participant_DSPy/avg_acc_diff_dspy.png}
    \caption{DSPy Average Improvement on ACC.}
    \label{fig:avg-acc-dspy-improvement}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.85\textwidth}
    \includegraphics[width=\linewidth]{Figures/Results/Participant_DSPy/avg_mse_diff_dspy.png}
    \caption{DSPy Average Improvement on MSE.}
    \label{fig:avg-mse-dspy-improvement}
  \end{subfigure}
  \caption{DSPy Average Improvement on ACC and MSE under different conditions.}
  \label{fig:average-acc-mse-dspy-improvement}
\end{figure}


\input{Tables/Participant-DSPy/participant-vs-dspy}



==> Sections/deleted/5-1-experimental-results.tex <==


\subsubsection{Participants Results}
\input{Sections/5-1-1-experimental-results-pure-participants}


\subsubsection{Participants with DSPy}
\input{Sections/5-1-2-experimental-result-with-DSPy}

==> Sections/deleted/5-2-Annotation-Process-Analysis.tex <==




==> Sections/deleted/5-3-Post-Lab-Analysis.tex <==






%---------------- dead kitten -------------------

\begin{comment}

\paragraph{Our system was helpful in prompt engineering} We asked participants to rate the satisfaction, helpfulness, and effectiveness of the system in the following questions: (i) How satisfied are you with the performance of the system? (ii) This tool was helpful in improving my prompt. (iii) Using this tool made the process of prompt engineering more efficient. These questions were rated on a seven-point Likert scale. Figure X shows the results. 

Overall, all participants expressed high satisfaction with our system's performance. They thought the system was helpful to improve prompts and make prompt engineering more efficient. 

% actual participant number starts from 103, I will use P1 to represent 103, P2->104...
Without our system, the typical approach to prompt engineering was varied. 
P1 made LLM assume it is a human and provided LLM with as much context as possible. 
Participants (P2, P4, P5) used a general refining process, starting prompts from scratch, testing prompts on data points, adjusting prompts based on incorrectly labeled data, re-testing, and re-verifying until the participant was satisfied. 

The post-questionnaire showed that our system also provided insights for participants on prompt engineering: ``adding or deleting a few words can change the overall output (P1)'', ``I can compare how many labels are correctly labeled before and after modifying prompts (P2)\steven{I rephrased participant's wording. is that ok}''...\steven{add more later}. 
One participant (P5) mentioned ``I really like this tool instead of traditional prompt engineering on Chatgpt and Copilot conversations.''

\end{comment}


==> Tables/Explanation/pure-participant-50-instances-detail.tex <==
\begin{table}[t]
    \centering
    \begin{threeparttable}
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
        \hline
         & \multicolumn{4}{c|}{\textbf{w/ 50 Instances} \tiny{(n=10)}} & \multicolumn{4}{c}{\textbf{w/o 50 Instances} \tiny{(n=10)}} \\
         \cmidrule(lr){2-5} \cmidrule(lr){6-9}
         & \multicolumn{2}{c|}{ACC$\uparrow$} & \multicolumn{2}{c|}{MSE$\downarrow$}& \multicolumn{2}{c|}{ACC$\uparrow$} & \multicolumn{2}{c}{MSE$\downarrow$}\\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
         & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{\%} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{\%}& \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{\%}& \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c}{\%}\\
         \hline
        \multicolumn{1}{l|}{\textbf{Start}} & \multicolumn{1}{c|}{.520} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{.742} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{.564} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{.822} & \multicolumn{1}{c|}{-}  \\
        \multicolumn{1}{l|}{\textbf{1st}}   & \multicolumn{1}{c|}{.530} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{.720} & \multicolumn{1}{c|}{40} & \multicolumn{1}{c|}{.542} & \multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{.870} & \multicolumn{1}{c|}{40}  \\
        \multicolumn{1}{l|}{\textbf{2nd}}   & \multicolumn{1}{c|}{.528} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{.780} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{.556} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{.886} & \multicolumn{1}{c|}{40}  \\
        \multicolumn{1}{l|}{\textbf{3rd}}   & \multicolumn{1}{c|}{.546} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{.722} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{.552} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{.924} & \multicolumn{1}{c|}{40}  \\
        \multicolumn{1}{l|}{\textbf{4th}}   & \multicolumn{1}{c|}{.536} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{.730} & \multicolumn{1}{c|}{40} & \multicolumn{1}{c|}{.570} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{.890} & \multicolumn{1}{c|}{40}  \\
        \hline
        \multicolumn{1}{l|}{End of Session} & \multicolumn{1}{c}{\multirow{2}{*}{.536}}& \multicolumn{1}{c}{\multirow{2}{*}{60}}& \multicolumn{1}{c}{\multirow{2}{*}{.736}}& \multicolumn{1}{c}{\multirow{2}{*}{40}}& \multicolumn{1}{c}{\multirow{2}{*}{.556}}& \multicolumn{1}{c}{\multirow{2}{*}{30}}& \multicolumn{1}{c}{\multirow{2}{*}{.894}}& \multicolumn{1}{c}{\multirow{2}{*}{50}}\\
        \multicolumn{1}{l|}{Avg \#Iter (4.75)}\\
        \hline
    \end{tabular}
    \begin{tablenotes}
        \tiny
        \item Avg: the average value of either ACC or MSE.
        \item \%: number of user improved ACC/MSE over ``Start'' $/$number of total user
    \end{tablenotes}
    \end{threeparttable}
    \caption{Participants' performance per iteration with or without 50 instances}
    \label{tab:participant-explanation-detail}
\end{table}


        
        
        % \multicolumn{1}{l}{\textbf{End of Session}} \\



 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}

==> Tables/Explanation/pure-participant-explanation-detail.tex <==
\begin{table}[t]
    \centering
    \begin{threeparttable}
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
        \hline
         & \multicolumn{4}{c|}{\textbf{w/ Explanation} \tiny{(n=10)}} & \multicolumn{4}{c}{\textbf{w/o Explanation} \tiny{(n=10)}} \\
         % & \multicolumn{4}{c|}{\tiny{(n=10)}} & \multicolumn{4}{c}{\tiny{(n=10)}}\\ 
         \cmidrule(lr){2-5} \cmidrule(lr){6-9}
         & \multicolumn{2}{c|}{ACC$\uparrow$} & \multicolumn{2}{c|}{MSE$\downarrow$}& \multicolumn{2}{c|}{ACC$\uparrow$} & \multicolumn{2}{c}{MSE$\downarrow$}\\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
         & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{\%} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{\%}& \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{\%}& \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c}{\%}\\
         \hline
        \multicolumn{1}{l|}{\textbf{Start}}  & \multicolumn{1}{c|}{.586} & \multicolumn{1}{c|}{-}  & \multicolumn{1}{c|}{.614} & \multicolumn{1}{c|}{-}& \multicolumn{1}{c|}{.498}& \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{.950}& \multicolumn{1}{c}{-}\\
        \multicolumn{1}{l|}{\textbf{1st}}    & \multicolumn{1}{c|}{.558} & \multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{.624} & \multicolumn{1}{c|}{40}& \multicolumn{1}{c|}{.514}& \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{.966} & \multicolumn{1}{c}{40}\\
        \multicolumn{1}{l|}{\textbf{2nd}}    & \multicolumn{1}{c|}{.570} & \multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{.632} & \multicolumn{1}{c|}{60}& \multicolumn{1}{c|}{.514}& \multicolumn{1}{c|}{60}& \multicolumn{1}{c|}{1.034} & \multicolumn{1}{c}{30}\\
        \multicolumn{1}{l|}{\textbf{3rd}}    & \multicolumn{1}{c|}{.560} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{.646} & \multicolumn{1}{c|}{50}& \multicolumn{1}{c|}{.538}& \multicolumn{1}{c|}{70}& \multicolumn{1}{c|}{1.000} & \multicolumn{1}{c}{50}\\
        \multicolumn{1}{l|}{\textbf{4th}}    & \multicolumn{1}{c|}{.556} & \multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{.646} & \multicolumn{1}{c|}{40}& \multicolumn{1}{c|}{.55}& \multicolumn{1}{c|}{70}& \multicolumn{1}{c|}{.974} & \multicolumn{1}{c}{40}\\
        \hline
        \multicolumn{1}{l|}{End of Session} & \multicolumn{1}{c}{\multirow{2}{*}{.556}}& \multicolumn{1}{c}{\multirow{2}{*}{20}}& \multicolumn{1}{c}{\multirow{2}{*}{.674}} & \multicolumn{1}{c}{\multirow{2}{*}{40}} & \multicolumn{1}{c}{\multirow{2}{*}{.536}} & \multicolumn{1}{c}{\multirow{2}{*}{70}} & \multicolumn{1}{c}{\multirow{2}{*}{.956}}& \multicolumn{1}{c}{\multirow{2}{*}{50}}\\
        \multicolumn{1}{l|}{Avg \#Iter (4.75} \\
        \hline
    \end{tabular}
    \begin{tablenotes}
        \tiny
        \item Avg: the average value of either ACC or MSE.
        \item \%: number of user improved ACC/MSE over ``Start'' $/$number of total user
    \end{tablenotes}
    \end{threeparttable}
    \caption{Participants' performance per iteration with or without LLM Explanation.}
    \label{tab:participant-explanation-detail}
\end{table}


        
        
        % \multicolumn{1}{l}{\textbf{End of Session}} \\



 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}

==> Tables/Participant-DSPy/participant-vs-dspy.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{l|cccccccccccc}
        \hline
         & \multicolumn{2}{c|}{\textbf{Human}} & \multicolumn{2}{c|}{\textbf{Human+DSPy}}& \multicolumn{2}{c|}{\textbf{Bootstrap}}& \multicolumn{2}{c|}{\textbf{Simple Prompt}}& \multicolumn{2}{c|}{\textbf{Mipro}}& \multicolumn{2}{c|}{\textbf{Copro}} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}  
         & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{MSE$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{MSE$\downarrow$}& \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{MSE$\downarrow$}& \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{MSE$\downarrow$}& \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{MSE$\downarrow$}& \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{MSE$\downarrow$}\\
         \hline
        \multicolumn{1}{l|}{\textbf{Start}} & \multicolumn{1}{c|}{0.542} & \multicolumn{1}{c|}{0.782} & \multicolumn{1}{c|}{-}& \multicolumn{1}{c|}{-}& \multicolumn{1}{c|}{-}& \multicolumn{1}{c|}{-}& \multicolumn{1}{c|}{-}& \multicolumn{1}{c|}{-}& \multicolumn{1}{c|}{-}& \multicolumn{1}{c|}{-}& \multicolumn{1}{c|}{-}& \multicolumn{1}{c|}{-}  \\
        \multicolumn{1}{l|}{\textbf{1st}}    & \multicolumn{1}{c|}{0.536}	 & \multicolumn{1}{c|}{0.795}	 & \multicolumn{1}{c|}{0.538}	 & \multicolumn{1}{c|}{0.889}	 & \multicolumn{1}{c|}{0.526}	 & \multicolumn{1}{c|}{0.915}	 & \multicolumn{1}{c|}{0.533}	 & \multicolumn{1}{c|}{0.864}	 & \multicolumn{1}{c|}{0.527}	 & \multicolumn{1}{c|}{0.973}	 & \multicolumn{1}{c|}{0.565}	 & \multicolumn{1}{c|}{0.822}   \\
        \multicolumn{1}{l|}{\textbf{2nd}}    & \multicolumn{1}{c|}{0.542}	 & \multicolumn{1}{c|}{0.833}	 & \multicolumn{1}{c|}{0.535}	 & \multicolumn{1}{c|}{0.883}	 & \multicolumn{1}{c|}{0.534}	 & \multicolumn{1}{c|}{0.934}	 & \multicolumn{1}{c|}{0.533}	 & \multicolumn{1}{c|}{0.864}	 & \multicolumn{1}{c|}{0.536}	 & \multicolumn{1}{c|}{0.862}	 & \multicolumn{1}{c|}{0.538}	 & \multicolumn{1}{c|}{0.873}   \\
        \multicolumn{1}{l|}{\textbf{3rd}}    & \multicolumn{1}{c|}{0.549}	 & \multicolumn{1}{c|}{0.823}	 & \multicolumn{1}{c|}{0.544}	 & \multicolumn{1}{c|}{0.847}	 & \multicolumn{1}{c|}{0.550}	 & \multicolumn{1}{c|}{0.850}	 & \multicolumn{1}{c|}{0.533}	 & \multicolumn{1}{c|}{0.864}	 & \multicolumn{1}{c|}{0.547}	 & \multicolumn{1}{c|}{0.873}	 & \multicolumn{1}{c|}{0.544}	 & \multicolumn{1}{c|}{0.801}  \\
        \multicolumn{1}{l|}{\textbf{4th}}    & \multicolumn{1}{c|}{0.553}	 & \multicolumn{1}{c|}{0.810}	 & \multicolumn{1}{c|}{0.537}	 & \multicolumn{1}{c|}{0.859}	 & \multicolumn{1}{c|}{0.526}	 & \multicolumn{1}{c|}{0.889}	 & \multicolumn{1}{c|}{0.533}	 & \multicolumn{1}{c|}{0.864}	 & \multicolumn{1}{c|}{0.536}	 & \multicolumn{1}{c|}{0.874}	 & \multicolumn{1}{c|}{0.554}	 & \multicolumn{1}{c|}{0.809}  \\
        \hline
        \multicolumn{1}{l|}{End of Session} & \multicolumn{1}{c}{\multirow{2}{*}{0.546}}& \multicolumn{1}{c}{\multirow{2}{*}{0.815}}& \multicolumn{1}{c}{\multirow{2}{*}{0.537}}& \multicolumn{1}{c}{\multirow{2}{*}{0.859}}& \multicolumn{1}{c}{\multirow{2}{*}{0.526}}& \multicolumn{1}{c}{\multirow{2}{*}{0.889}}& \multicolumn{1}{c}{\multirow{2}{*}{0.533}}& \multicolumn{1}{c}{\multirow{2}{*}{0.864}} & \multicolumn{1}{c}{\multirow{2}{*}{0.536}}& \multicolumn{1}{c}{\multirow{2}{*}{0.874}}& \multicolumn{1}{c}{\multirow{2}{*}{0.554}}& \multicolumn{1}{c}{\multirow{2}{*}{0.809}}\\
        \multicolumn{1}{l|}{Avg \#Iter (4.75)}\\
        \hline
    \end{tabular}
    \caption{Average Performance per iteration for Participants, Participant plus DSPy, and four different DSPy algorithms.}
    \label{tab:participant-explanation-detail}
\end{table}


        
        
        % \multicolumn{1}{l}{\textbf{End of Session}} \\



 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}
 % & \multicolumn{1}{c|}{}

==> Tables/acc-improvement.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lccccc|cccccc}
        \hline
        \multicolumn{1}{l} {ACC Change}  & \multicolumn{5}{c|}{\textbf{50Y}} & \multicolumn{5}{c}{\textbf{50N}} &\multicolumn{1}{c}{Perf. Change}
        \\ \cmidrule(lr){2-6} \cmidrule(lr){7-11} 
        \multicolumn{1}{l}{\textbf{LY}} & \multicolumn{5}{c}{(-.020) 2 $\uparrow$ \hspace{0.2cm} 2 $\downarrow$ \hspace{0.2cm} 1 $\leftrightarrow$} & \multicolumn{5}{c}{(-.040) 0 $\uparrow$ \hspace{0.2cm} 5 $\downarrow$ \hspace{0.2cm} 0 $\leftrightarrow$} &\multicolumn{1}{c}{(-.030) 2 $\uparrow$ \hspace{0.2cm} 7 $\downarrow$ \hspace{0.2cm} 1 $\leftrightarrow$}\\ 
        \hline
        \multicolumn{1}{l}{\textbf{LN}}  & \multicolumn{5}{c}{\underline{\textbf{(.052) 4 $\uparrow$ \hspace{0.2cm} 1 $\downarrow$ \hspace{0.2cm} 0 $\leftrightarrow$}}}& \multicolumn{5}{c}{(.052) 3 $\uparrow$ \hspace{0.2cm} 2 $\downarrow$ \hspace{0.2cm} 0 $\leftrightarrow$}  &\multicolumn{1}{c}{(.052) 7 $\uparrow$ \hspace{0.2cm} 3 $\downarrow$ \hspace{0.2cm} 0 $\leftrightarrow$} \\ 
        \bottomrule
        \multicolumn{1}{l}{{Perf. Change}}  & \multicolumn{5}{c}{(.016) 6 $\uparrow$ \hspace{0.2cm} 3 $\downarrow$ \hspace{0.2cm} 1 $\leftrightarrow$} & \multicolumn{5}{c}{(.006) 3 $\uparrow$ \hspace{0.2cm} 7 $\downarrow$ \hspace{0.2cm} 0 $\leftrightarrow$}
        \\
    \end{tabular}
    \caption{The result of Accuracy Improvements. Participants under \textbf{LN} achieves the highest accuracy improvement of 0.052 over all conditions. Participants under both \textbf{LN and 50Y} have the most individual improving their labeling accuracy. The bold and underline combination is the best across all conditions.}
    \label{tab:acc-improvement}
\end{table}

==> Tables/data-annotation-survey-questions.tex <==
\begin{table*}
\footnotesize
\centering
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{\#} & \textbf{Aspect} & \textbf{Questionnaire Question} \\ \midrule
Q1 & Basic Information & \begin{tabular}[c]{@{}l@{}}What is the best description(s) for your role in the data labeling process? \\(1) Data Scientist (2) Researcher
(3) Project Manager
(4) Machine Learning Engineer
(5) Software Engineer
(6) Student\\
(7) Crowd Workers
(8) Other\end{tabular} \\ \midrule
Q2 & Basic Information & \begin{tabular}[c]{@{}l@{}}The annotation tool is easy to use.\\
(1) Technology/IT
(2) Finance
(3) Education
(4) Manufacturing
(5) Retail/E-commerce
(6) Government/Public Sector\\
(7) Research and Development
(8) Other
\end{tabular} \\ \midrule
Q3 & Basic Information & \begin{tabular}[c]{@{}l@{}}What is your years of experience in data labeling?\\
(1) Less than 1 year
(2) 1-3 years
(3) 4-6 years
(4) More than 6 years
 \end{tabular} \\ \midrule
Q4 & Basic Information & \begin{tabular}[c]{@{}l@{}}What is your years of experience in using LLMs to do data labeling?
 \\
(1) Less than a month
(2) 1-3 months
(3) 4 months to 1 year
(4) More than 1 year
 \end{tabular} \\ \midrule
Q5 & Basic Information & \begin{tabular}[c]{@{}l@{}}What types of data do you primarily work with in your role? \\
(1) Text
(2) Images
(3) Audio
(4) Video
(5) Sensor data (e.g., IoT)
(6) Multimodal data
(7) Other
\end{tabular} \\ \midrule
Q6 & Basic Information & \begin{tabular}[c]{@{}l@{}}How often do you use LLMs to assist any step in annotation tasks (e.g. for prompting, labeling, verification, etc)? \\
(1) Daily
(2) Weekly
(3) Bi-Weekly
(4) Monthly
(5) Never
\end{tabular} \\ \midrule
Q7 & Basic Information & \begin{tabular}[c]{@{}l@{}}What is the following best describe your process of using LLMs to data labeling?
 \\
(1) I use LLMs for an initial pass of labeling, then review and revise the labels myself.\\
(2) I manually label the data (or obtain labels from others) first and use LLMs to validate or review the labels.\\
(3) I consult LLMs for ambiguous cases or to resolve disagreements.\\
(4) I use LLMs for data pre-processing, such as transforming unstructured text into structured data.\\
(5) I use LLMs to generate task-based examples for creating additional data.\\
(6) I use LLMs to provide explanations for some labeled data.\\
(7) Other\\
 \end{tabular} \\ \midrule
Q8 & Creating Prompting & \begin{tabular}[c]{@{}l@{}}Please provide a brief description of your typical annotation process with an LLM.\\
\textit{Walk us through your steps, from initializing the task to reviewing and finalizing annotations. Include any strategies you use}\\ \textit{to ensure quality or consistency.}\end{tabular} \\ \midrule
Q9 & Creating Prompting & \begin{tabular}[c]{@{}l@{}}How do you typically initialize the annotation process with an LLM?\\
\textit{For example, do you start with predefined prompts, or do you ask the LLM for suggestions?}\end{tabular} \\ \midrule
Q10 & Creating Prompting & \begin{tabular}[c]{@{}l@{}}Please describe your process for revising prompts when using an LLM for annotation.\\
\textit{For example, how do you refine or adjust prompts to achieve the desired response? How do you handle bias or inconsistencies}\\ \textit{introduced by the LLM in your annotations?} \end{tabular} \\ \midrule
Q11 & Creating Prompting & \begin{tabular}[c]{@{}l@{}}How much time do you spend crafting and refining prompts for each annotation task?\\
(1) Less than 5 minutes
(2) 5-10 minutes
(3) 10-15 minutes
(4) More than 15 minutes
\end{tabular} \\ \midrule
Q12 & Process Prompting Response & \begin{tabular}[c]{@{}l@{}}Which of the following best describes your manual review efforts when working with LLM-generated labels?\\
(1) I rely on all LLM-generated labels.\\
(2) I only review labels for randomly sampled subset/ critical tasks/ specific use /ambiguous cases.\\
(3) I cross-check LLM-generated labels against established guidelines or standards.\\
(4) I compare LLM-generated labels with expert-provided labels for validation.\\
(5) I manually verify all LLM-generated labels for accuracy and consistency.\\
(6) I use LLM-generated labels as a starting point and fully revise them as needed.\\
(7) I collaborate with domain experts to evaluate and refine LLM-generated labels.\\
(8) Other\\
\end{tabular} \\ \midrule
Q13 & Process Prompting Response & \begin{tabular}[c]{@{}l@{}}When the label explanation is provided, please describe how you use LLM's explanation in your annotation tasks.
\end{tabular} \\ \midrule
Q14 & Process Prompting Response & \begin{tabular}[c]{@{}l@{}}As of November 2024, how reliable do you find LLMs for generating accurate annotations?\\
(1) Very reliable
(2) Somewhat Reliable
(3) Neutral
(4) Somewhat Unreliable
(5) Very unreliable
\end{tabular} \\ \midrule
Q15 & Process Prompting Response & \begin{tabular}[c]{@{}l@{}}How has using an LLM impacted your annotation speed?\\
(1) Greatly increased
(2) Slightly increased
(3) No change
(4) Slightly decreased
(5) Greatly decreased
\end{tabular} \\ \midrule
Q16 & Process Prompting Response & \begin{tabular}[c]{@{}l@{}}What impact has using an LLM had on the quality of your annotations?\\
(1) Greatly increased
(2) Slightly increased
(3) No change
(4) Slightly decreased
(5) Greatly decreased
\end{tabular} \\ \midrule
Q17 & Annotation Validation and Gold Labels & \begin{tabular}[c]{@{}l@{}}How do you validate LLM-assisted annotations?
\end{tabular} \\ \midrule
Q18 & Annotation Validation and Gold Labels& \begin{tabular}[c]{@{}l@{}}How often do you have gold-standard labels (either by you, other people, or experts) at the beginning of the annotation\\ process?\\
(1) 0–20\%
(2) 20–40\%
(3) 40–60\%
(4) 60–80\%
(5) 80–100\%
\end{tabular} \\ \midrule
Q19 & Annotation Validation and Gold Labels & \begin{tabular}[c]{@{}l@{}}What is the source of the gold-standard labels? If the gold-standard labels are not available or limited, how do you create\\ gold-standard labels? \end{tabular} \\ \midrule
Q20 & Annotation Validation and Gold Labels & \begin{tabular}[c]{@{}l@{}}How do you use gold-standard labels during the annotation process besides validation?\end{tabular} \\ 
\\ \bottomrule
\end{tabular}
\caption{Survey questions used for understanding how individuals use LLMs in data annotation.}
\label{tab:study-survey-annotation}
% \vspace{-5mm}
\end{table*}


==> Tables/dspy-t-test/dspy-t-test-detail-conditions-under-each-optimizer.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{lcccc|cccc}
        \hline
        \multicolumn{1}{l} {DSPy} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{ACC$\uparrow$}}} & \multicolumn{3}{c|}{\textbf{T-Test over Avg. Changed ACC}}& \multicolumn{1}{c}{\multirow{2}{*}{\textbf{MSE$\downarrow$}}} & \multicolumn{3}{c}{\textbf{T-Test over Avg. Changed MSE}}
        \\ \cmidrule(lr){3-5} \cmidrule(lr){7-9} 
        \multicolumn{1}{l} {Changes} & & LY-50N & LN-50Y & LN-50N & & LY-50N & LN-50Y & LN-50N\\
        \hline
        \textbf{Bootstrap}\\
        \cmidrule(lr){1-9}
        LY-50Y & .004 & .335&.083&.011*      & .128 &  .903&.043*&.049*   \\ \hline
        LY-50N  & -.014 & -      & .025 & .109     & .119 & -      & .236&.217   \\ \hline
        LN-50Y  & \underline{.039} & -      & -    & <.001***       & .018 & -      & -    & .893   \\ \hline
        LN-50N   & -.055 & -      & -    & -           & .009 & -      & -    & -      \\ 
        \midrule
        \textbf{Simple Prompt}\\
        \cmidrule(lr){1-9}
        LY-50Y & -.003 & .564&.076&.002**      & .179 &  .045*&.034*&.002**   \\ \hline
        LY-50N  & .009 & -      & .129 & <.001***     & .035 & -      & .630&.219   \\ \hline
        LN-50Y  & \textbf{.041} & -      & -    & <.001***       & .073 & -      & -    & .070   \\ \hline
        LN-50N   & -.095 & -      & -    & -           & \underline{-.092} & -      & -    & -      \\ 
        \midrule
        \textbf{Mipro}\\
        \cmidrule(lr){1-9}
        LY-50Y & .029 & .040*&.826&.010**      & .094 &  .651&.025*&.261   \\ \hline
        LY-50N  & -.014 & -      & .079&.195     & .124 & -      & .026*&.188   \\ \hline
        LN-50Y  & .035 & -      & -    & .015*       & -.048 & -      & -    & .557   \\ \hline
        LN-50N   & -.056 & -      & -    & -           & .003 & -      & -    & -      \\ 
        \midrule
        \textbf{Copro}\\
        \cmidrule(lr){1-9}
        LY-50Y & .021 & .137&.651&.095      & .052 &  .436&.052&.024*   \\ \hline
        LY-50N  & -.006 & -      & .137&.774     & .098 & -      & .044*&.017*   \\ \hline
        LN-50Y  & .031 & -      & -    & .098       & -.046 & -      & -    & .443   \\ \hline
        LN-50N   & -.012 & -      & -    & -           & \textbf{-.104} & -      & -    & -      \\ 
        \hline
    \end{tabular}
    \caption{DSPy t-test over different conditions for each optimizer.\kenneth{Did we even mention Table 5 in the paper????? Maybe just remove it.}}
    \label{tab:dspy-all-conditions-t-test}
\end{table}



==> Tables/dspy-t-test/dspy-t-test-general-condition.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lcccc|cccc}
        \hline
        \multicolumn{1}{l} {DSPy} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{ACC$\uparrow$}}} & \multicolumn{3}{c|}{\textbf{T-Test over Avg. Changed ACC}}& \multicolumn{1}{c}{\multirow{2}{*}{\textbf{MSE$\downarrow$}}} & \multicolumn{3}{c}{\textbf{T-Test over Avg. Changed MSE}}
        \\ \cmidrule(lr){3-5} \cmidrule(lr){7-9} 
        \multicolumn{1}{l} {Changes} & & LY-50N & LN-50Y & LN-50N & & LY-50N & LN-50Y & LN-50N\\
        \hline
        LY-50Y & .012 & .060 & .033* & <.001***      & .114 &  .520  & <.001*** & <.001**   \\ \hline
        LY-50N  & -.006 & -      & <.001*** & <.001***     & .092 & -      & .020* & .002**   \\ \hline
        LN-50Y  & .036 & -      & -    & <.001***       & .003 & -      & -    & .215   \\ \hline
        LN-50N   & -.054 & -      & -    & -           & -.047 & -      & -    & -      \\ \hline
    \end{tabular}
    \caption{DSPy t-test over different conditions for all optimizers.}
    \label{tab:dspy-general-conditions-t-test}
\end{table}



==> Tables/kappa/kappa-detail.tex <==
\begin{table}[h]
\begin{tabular}{l|cccc}
Kappa & \multicolumn{1}{l}{Original Avg} & \multicolumn{1}{l}{Std} & \multicolumn{1}{l}{Each Participant Avg} & \multicolumn{1}{l}{Std} \\
\hline
\multicolumn{1}{l|}{LY}    & 0.098 & 0.057    & \textbf{0.333}& 0.039    \\
\multicolumn{1}{l|}{LN}   & 0.129             & 0.081    & 0.193&0.047    \\
\multicolumn{1}{l|}{50Y}   & \textbf{0.135}             & 0.073    & 0.263&	0.049    \\
\multicolumn{1}{l|}{50N}  & 0.092             & 0.062    & 0.220& 0.060             \\
\bottomrule
\end{tabular}
\caption{Kappa for each condition. Original Avg refers to the average Kappa score between each participant and the original dataset. Each Participant Avg represents the average of the mean Kappa values for each participant compared to the others under the same condition.}
    \label{tab:kappa-detail}
\end{table}

==> Tables/mixed-condition-t-test.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lcccc|cccc}
        \hline
        \multicolumn{1}{l} {Eval} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{ACC}}} & \multicolumn{3}{c|}{\textbf{T-Test over Avg. ACC}}& \multicolumn{1}{c}{\multirow{2}{*}{\textbf{MSE}}} & \multicolumn{3}{c}{\textbf{T-Test over Avg. MSE}}
        \\ \cmidrule(lr){3-5} \cmidrule(lr){7-9} 
        \multicolumn{1}{l} {Condition} & & LY-50N & LN-50Y & LN-50N & & LY-50N & LN-50Y & LN-50N\\
        \hline
        LY-50Y & 0.566 & .441   & .001** & .855      & \textbf{0.556} &  .135  & <.001*** & .025*   \\ \hline
        LY-50N  & \textbf{0.582} & -      & .001** & .473     & 0.682 & -      & .019* & .086   \\ \hline
        LN-50Y  & 0.498 & -      & -    & .033*       & 0.922 & -      & -    & .435   \\ \hline
        LN-50N   & 0.561 & -      & -    & -           & 1.105 & -      & -    & -      \\ \hline
    \end{tabular}
    \caption{The result of mixed condition Accuracy and MSE. LN-50Y has significantly lower accuracy than the rest of the combinations. LY-50Y has a significantly better MSE than participants who have LN conditions. }
    \label{tab:mixed-condition-t-test}
\end{table}



==> Tables/mse-improvement.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lccccc|cccccc}
        \hline
        \multicolumn{1}{l} {MSE Change}  & \multicolumn{5}{c|}{\textbf{50Y}} & \multicolumn{5}{c}{\textbf{50N}} &\multicolumn{1}{c}{Perf. Change}
        \\ \cmidrule(lr){2-6} \cmidrule(lr){7-11} 
        \multicolumn{1}{l}{LY} & \multicolumn{5}{c}{(-.004) 2 $\uparrow$ \hspace{0.2cm} 2 $\downarrow$ \hspace{0.2cm} 1 $\leftrightarrow$} & \multicolumn{5}{c}{(.068) 2 $\uparrow$ \hspace{0.2cm} 3 $\downarrow$ \hspace{0.2cm} 0 $\leftrightarrow$} &\multicolumn{1}{c}{ (.032)  4 $\uparrow$ \hspace{0.2cm} 5 $\downarrow$ \hspace{0.2cm} 1 $\leftrightarrow$}\\ 
        \hline
        \multicolumn{1}{l}{LN}  & \multicolumn{5}{c}{\underline{\textbf{(-.020) 2 $\uparrow$ \hspace{0.2cm} 2 $\downarrow$ \hspace{0.2cm} 1 $\leftrightarrow$}}}& \multicolumn{5}{c}{(.068) 2 $\uparrow$ \hspace{0.2cm} 3 $\downarrow$ \hspace{0.2cm} 0 $\leftrightarrow$}  &\multicolumn{1}{c}{(.024)  4 $\uparrow$ \hspace{0.2cm} 5 $\downarrow$ \hspace{0.2cm} 1 $\leftrightarrow$} \\ 
        \bottomrule
        \multicolumn{1}{l}{{Perf. Change}}  & \multicolumn{5}{c}{(-.012) 4 $\uparrow$ \hspace{0.2cm} 4 $\downarrow$ \hspace{0.2cm} 2 $\leftrightarrow$} & \multicolumn{5}{c}{(.068) 4 $\uparrow$ \hspace{0.2cm} 6 $\downarrow$ \hspace{0.2cm} 0 $\leftrightarrow$}
        \\
    \end{tabular}
    \caption{The result of MSE Improvements. Participants under LN and 50Y achieves the greatest MSE improvement, with a reduction of 0.020. Participants under 50Y had a slightly better MSE improvement than those with 50N. The bold and underline combination is the best across all conditions.}    \label{tab:mse-improvement}
\end{table}

==> Tables/ovearll-participant-result-table-1-backup.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lcccc}
 & \multicolumn{2}{c}{\textbf{ACC}} & \multicolumn{2}{c}{\textbf{MSE}} \\ \hline
\multicolumn{1}{c}{} & \textbf{Avg.} & \textbf{\begin{tabular}[c]{@{}c@{}}\%Participant\\ Improved\\ Over Initial\end{tabular}} & \textbf{Avg.} & \textbf{\begin{tabular}[c]{@{}c@{}}\%Participant\\ Improved\\ Over Initial\end{tabular}} \\ \hline
\textbf{Starting Prompt} & .542 (SD=.099) & - & .782 (SD=.482) & - \\ \hline
\textbf{1st Revision} & .536 (SD=.088) & 35\% & .795 (SD=.546) & 40\% \\
\textbf{2nd Revision} & .542 (SD=.073) & 40\% & .833 (SD=.514) & 45\% \\
\textbf{3rd Revision} & .549 (SD=.082) & 50\% & .823 (SD=.579) & 50\% \\
\textbf{4th Revision} & .553 (SD=.085) & 45\% & .810 (SD=.566) & 40\% \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}End of Session\\ (Avg \#Iter = 4.75)\end{tabular}} & .546 (SD=.084) & 45\% & .815 (SD=.489) & 45\%
\end{tabular}
\caption{\kenneth{TODO: For the overall results, add a table}\steven{done, should we change it to the same format as the later tables?}}
\label{tab:overall-ACC-MSE}
\end{table}

==> Tables/single-condition-t-test-acc.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lcccc}
        \hline
        \multicolumn{1}{l} {Eval} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{ACC}}} & \multicolumn{3}{c}{\textbf{T-Test over Avg. ACC}}
        \\ \cmidrule(lr){3-5} 
        \multicolumn{1}{l} {Condition} & & LLM-No & 50-Yes & 50-No\\
        \hline
        LLM-Yes & \textbf{.573} & .009**   & .007** & .937   \\ \hline
        LLM-No  & .526 & -      & .752 & .029*   \\ \hline
        50-Yes  & .532 & -      & -    & .033*   \\ \hline
        50-No   & .572 & -      & -    & -      \\ \hline
    \end{tabular}
    \caption{The result of single condition accuracy. LLM-Yes has significantly higher accuracy than LLM-No and 50-Yes conditions.}
    \label{tab:single-condition-acc}
\end{table}

==> Tables/single-condition-t-test-mse.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lcccc}
        \hline
        \multicolumn{1}{l} {Eval} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{MSE}}} & \multicolumn{3}{c}{\textbf{T-Test over Avg. MSE}}
        \\ \cmidrule(lr){3-5} 
        \multicolumn{1}{l} {Condition} & & LLM-No & 50-Yes & 50-No\\
        \hline
        LLM-Yes & 0.613 & <.001***   & .023* & .033*   \\ \hline
        LLM-No  & 1.000 & -      & .020* & .502   \\ \hline
        50-Yes  & 0.739 & -      & -    & .230   \\ \hline
        50-No   & 0.895 & -      & -    & -      \\ \hline
    \end{tabular}
    \caption{The result of single condition MSE. LLM-Yes has significantly lower MSE than the rest of the conditions.}
    \label{tab:single-condition-mse}
\end{table}

==> Tables/single-condition-t-test.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lcccc|cccc}
        \hline
        \multicolumn{1}{l} {Eval} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{ACC}}} & \multicolumn{3}{c|}{\textbf{T-Test over Avg. ACC}}& \multicolumn{1}{c}{\multirow{2}{*}{\textbf{MSE}}} & \multicolumn{3}{c}{\textbf{T-Test over Avg. MSE}}
        \\ \cmidrule(lr){3-5} \cmidrule(lr){7-9} 
        \multicolumn{1}{l} {Condition} & & LN & 50Y & 50N & & LN & 50Y & 50N\\
        \hline
        LY & \textbf{0.573} & .009**   & .007** & .937& \textbf{0.613} & <.001***   & .023* & .033*   \\ \hline
        LN  & 0.526 & -      & .752 & .029*  & 1.000 & -      & .020* & .502   \\ \hline
        50Y  & 0.532 & -      & -    & .033*  & 0.739 & -      & -    & .230   \\ \hline
        50N   & 0.572 & -      & -    & -    &   0.895 & -      & -    & -      \\ \hline
    \end{tabular}
    \caption{The result of single condition Accuracy and MSE. LY has significantly higher accuracy than LN and 50Y conditions; LY has significantly lower MSE than the rest of the conditions. The p-values were calculated by comparing accuracy or MSE across all participants in each condition (*:p<0.05; **:p<0.01; ***:p<0.001; independent t-test.) }
    \label{tab:single-condition-t-test}
\end{table}


